Efficient Neural Architecture Search via Parameter Sharing

We propose Efficient Neural Architecture Search (ENAS), a fast and inexpensive approach for automatic model design. In ENAS, a controller learns to discover neural network architectures by searching for an optimal subgraph within a large computational graph. The controller is trained with policy gradient to select a subgraph that maximizes the expected reward on the validation set. Meanwhile the model corresponding to the selected subgraph is trained to minimize a canonical cross entropy loss. Thanks to parameter sharing between child models, ENAS is fast: it delivers strong empirical performances using much fewer GPU-hours than all existing automatic model design approaches, and notably, 1000x less expensive than standard Neural Architecture Search. On the Penn Treebank dataset, ENAS discovers a novel architecture that achieves a test perplexity of 55.8, establishing a new state-of-the-art among all methods without post-training processing. On the CIFAR-10 dataset, ENAS designs novel architectures that achieve a test error of 2.89%, which is on par with NASNet (Zoph et al., 2018), whose test error is 2.65%.

==> bayesian.tex <==
\section{\label{sec:bayes}A Bayesian Framework}

We briefly review the relevant background in Bayesian neural networks and two
variational inference methods, specifically mean-field approximation and
structured approximation. We the proceed to show that NAS can be casted as an
instance of Bayesian neural networks and that this formulation of NAS inspires
our novel approach.

\subsection{\label{sec:bayesian}The Bayesian Framework}
Suppose we want to model an unknown distribution $p(\x)$ of our data. In the
Bayesian framework~\citep{bayes_nn}, we seek to learn a latent variable $\z$ in
the probability space $Z$ such that $z$ is likely to generate our data $\x$. We
start by postulating a prior distribution $p(\z)$ over the possible hidden
variables $\z$, which represents our initial belief in how $z$ should look
like. We then attempt to learn a distribution $q(\z)$ over $\Z$ that minimizes
the Kullback-Leiber divergence between $q(\z)$ and the true posterior $p(\z |
\x)$. Using Bayes rule, we can write the KL divergence as follows.
\begin{align}
  \text{KL}\left( q(\z) \parallel p(\z | \x) \right)
    &= \mathbb{E}_{\z \sim q} \left[ \log{q(\z)} \right]
     - \mathbb{E}_{\z \sim q} \left[ \log{p(\x | \z)} \right]
     - \mathbb{E}_{\z \sim q} \left[ \log{p(\z)} \right] + \log{p(\x)} \\
    &= -\mathbb{E}_{\z \sim q} \left[ \log{p(\x | \z)} \right]
     + \mathbb{E}_{\z \sim q}\left[ \log{q(\z)} - \log{p(\z)} \right] + \log{p(\x)} \\
    \label{eqn:elbo}
    &\leq -\mathbb{E}_{\z \sim q} \left[ \log{p(\x | \z)} \right] + \text{KL}(q(\z) \parallel p(\z))
\end{align}
The right-hand side of Eqn~\ref{eqn:elbo} is called the \textit{Evidence Lower
Bound} (ELBO) of the hypothesized distribution $q(\z)$. The ELBO captures the
expected log-likelihood $\mathbb{E}_{z \sim q} \left[ \log{p(\x | \z)} \right]$
of the data $\x$ given the latent variable $\z$, which we can observe from our
training data. In recent work, the divergence $\text{KL}(q(\z) \parallel
p(\z))$ was treated as a regularization term. For
instance,~\cite{variational_dropout,variational_dropout_rnn} approximated the
KL divergence with an $\ell_2$ regularization on their parameters, equivalently
assuming a prior $p(\z)$ to put weights on the all parameters being $0$. The
take-away message is that in practice, one can approximate the ELBO term in
different ways, leading to different learning algorithms.

\subsection{\label{sec:mean_field_and_structured}Mean-field and Structured Variational Approximation}
If the latent variable $\z$ can take on an arbitrary form, then the ELBO term
is intractable. Mean-field approximation relaxes all the dependencies among
components of $\z$. Specifically, mean-field approximation assumes that if $\z
= (z_1, z_2, ..., z_m)$ then
\begin{align}
  q(\z) = \prod_{i=1}^{m} q_i(z_i)
\end{align}
While such independence assumption makes it easier to learn $q(\z)$, it
introduces a bias in the space of latent variables $\Z$. This is because the
true posterior $p(\z | \x)$, which we aim to approximate with $q(\z)$, may have
a degree of dependencies between the components $z_i$'s. In contrast to
mean-field approximiation,structured variational approximation
methods~\citep{struct_approx} assume a certain degree of dependencies on the
components of $\z$, leading to a model with a higher fidelity to the true
posterior $p(\z | \x)$, at the tradeoff of more complex learning problem.

\subsection{\label{sec:bayesian_nas}Connection to Neural Architecture Search}
In~\cite{variational_inference_reviews}, it is noted that the ELBO
can be used as a criterion for model selection, effectively drawing a
connection from variational methods to NAS methods, which aim to select the
best models, a.k.a.  network architectures.

To cast the NAS problem as an instance of the described Bayesian framework, we
let $\z$ be a pair $(\m, \theta_{\m})$ of an architecture $\m$ and its
parameters $\theta_{\m}$, and note that $\m$ is a discrete latent variable. Now
we can write
\begin{align}
  \text{ELBO}(q)
    &= -\mathbb{E}_q \left[ \log{p(\x | \z)} \right]
     + \text{KL}(q(\m, \theta_\m) \parallel p(\m, \theta_\m | \x)) \\
    \label{eqn:models_and_params}
    &= -\sum_{\m} q(\m) \int{\log{p(\x | \m, \theta_\m)} q(\theta_{\m} | \m) d\theta_{\m}}
     + \text{KL}(q(\m, \theta_\m) \parallel p(\m, \theta_\m | \x))
\end{align}
Eqn.~\ref{eqn:models_and_params} exhibits an instance of structured variational
approximation as described in Section~\ref{sec:mean_field_and_structured}, as
$\theta_\m$ depends on $\m$ and has to be learned to fit with each model $\m$.
Some existing approaches for NAS falls into this
category~\citep{nas,nas_module,nas_dqn,nas_module_dqn}. As noted, structured
variational approximation has a high fidelity to the true posterior, which
means that the aforementioned methods can better approximate the true posterior
$p(\x | \z)$, at the cost of solving a more difficult learning problem. In the
case of NAS, the learning problem is to learn the parameters $\theta_\m$, which
means to optimize a neural network $\m$ from scratch. This is an expensive
process, and it leads to the notorious computational expense of these NAS
approaches.

On the other hand, mean-field variational approximation seems inappropriate for
NAS, because not all models $\m$ can be compatible with the parameters
$\theta_{\m'}$ of another model, e.g. the number of parameters can differ, not
to mention further structures in $\theta_\m$. However, in
Section~\ref{sec:enas}, we show that we are able to enforce a novel structure
on $\theta_\m$ which leads to a succesful mean-field approximation of
Eqn.~\ref{eqn:models_and_params}.

==> figs/intro.tex <==
\section{\label{sec:intro}Introduction}

Neural architecture search (NAS) has been applied successfully to design model
architectures for image classification and language
modeling~\citep{nas,nas_dqn,bello2017neural,nas_module,nas_by_transformation}.
NAS however is computationally expensive and time consuming: for
example,~\cite{nas_module} use $450$ GPUs and train for $3$-$4$ days.
Meanwhile, using less resources tends to produce less compelling
results~\citep{deep_arc,nas_dqn}.

%Although less resource-intensive alternatives to NAS exist, these alternatives produce less compelling results~\citep{deep_arc,nas_dqn}.

The main computational bottleneck of NAS is the training of each child model to
convergence to measure its accuracy. We believe that it is very inefficient and
wasteful to train every child model and then throw away all the trained weights
even though the child models have much in common.

\begin{figure}[H]
  \centering
  \includegraphics[width=0.45\textwidth]{figs/enas_dag.eps}
  \caption{The graph represents the entire search space while the red arrows
    define a model in the search space, which is decided by a controller.  Here
    we assume that node $1$ is the input to the model whereas nodes $3$, $5$,
    and $6$ are the outputs of the model.
  }
  \label{fig:enas_dag}
\end{figure}


The goal of this work is to remove this inefficiency by enabling more sharing
between the child models. This idea is similar to the concept of weight
inheritance in neuro-evolution (e.g.,~\cite{Real17}). To understand our method,
we first need to understand the standard NAS. In standard
NAS~\citep{nas,nas_dqn}, an RNN controller is trained by policy gradient to
search for a good architecture, which is basically a computational graph. Our
observation is that all of the graphs, that NAS has iterated over, can be
viewed as sub-graphs of a larger graph. In other words, we can represent the
space of these graphs as a \emph{single} directed acyclic graph (DAG). As
illustrated in Figure~\ref{fig:enas_dag}, a neural network architecture can be
found by taking a subset of edges in this DAG. This design is advantageous
because  it enables sharing parameters among all architectures in the search
space. %This design hence avoids the need to train from scratch every new
architecture found during the search process. 

Our method requires the training of a path within a large model together with the controller. The controller is trained with policy gradient to select a path that maximizes the expected reward on the validation set. Meanwhile the model corresponding to the selected path is trained to minimize a cross-entropy loss. In view of its efficiency, we name our method \textit{Efficient Neural Architecture Search} (\enasnospace).

ENAS is both theoretically sound and empirically efficient. Using Lyapunov functions~\citep{martingale_technique}, we can show that the training of \enas converges almost surely. Empirically, on CIFAR-10, \enas achieves the error rate of $2.89\%$, compared to $2.65\%$ by NAS. On Penn Treebank, \enas discovers an architecture that achieves the perplexity of $57.8$, which outperforms NAS's perplexity of $62.4$~\citep{nas}. In all of our experiments, \enas takes less than $16$ hours to train, whilst running on a single Nvidia GTX 1080Ti GPU. Compared to NAS, our method achieves a 10X reduction of search time and 100X reduction of computational resources.


==> figs/related.tex <==
%\section{\label{sec:related}Related Work}

\section{\label{sec:nas}Related Work}
%The goal of NAS is to find a model architecture $\m$ that achieves a high reward $R(\m)$ on a particular task. Recent approaches such as~\citet{nas,nas_module,nas_dqn,bello2017neural,nas_module_dqn} used reinforcement learning to search the combinatorial space of architectures, attempting to model a parameterized policy $\pi(\m; \theta)$ of $\m$ to maximize the expected reward $J(\theta) = \mathbb{E}_{\m \sim \pi(\m; \theta)} \left[ R(\m) \right]$.

%There are two main approaches for designing the search space. The first approach, which we call \emph{macro search space design}, designs the whole architecture all at once. For instance, if we were to design a convolutional network, we would choose how many filters to use at each layer, the filter sizes, how to set up the skip connections, etc. Macro design is used by~\cite{nas,nas_dqn,deep_arc,smash_net,conv_fabrics}. The second approach, which we call \emph{micro search space design}, aims to search for smaller modules which are then replicated and assembled to form the final model. Micro design is used by~\cite{nas_module,nas_module_dqn}. We note that~\cite{nas} also use micro design when designing the RNN cell.

%An architecture $\m$ is often represented as a sequence, with a grammar and meaning specified by the NAS algorithm.  Because modeling variable length sequences is necessary, the reinforcement learning policy $\pi(\m; \theta)$ is often parametrized with a recurrent neural network. $J(\theta)$ is then learned with various reinforcement learning algorithms such as REINFORCE~\citep{nas,reinforce}, Proximal Policy Optimization~\citep{nas_module,ppo}, and Q-learning~\citep{nas_dqn,nas_module_dqn}.

%NAS methods are typically time consuming and computationally expensive. Most significantly,~\cite{nas} and~\cite{nas_module} respectively train in $3$-$4$ weeks and $3$-$4$ days, using $800$ and $450$ GPUs concurrently at any time during their training. A summary from previous NAS approaches can be found in Table~\ref{tab:cifar10_times} in Appendix~\ref{sec:cifar10_details}. Such computational expense of NAS methods is due to the fact that each architecture $\m$ is trained from scratch to compute $R(\m)$. After training $\m$, only the reward $R(\m; \omega^{\text{opt}}_\m)$ is utilized, while the learned parameters of $\omega^{\text{opt}}_\m$, which could be reused, are thrown away.

There is growing interest in improving the efficiency of neural architecture search. Concurrent to our work are the promising ideas of using learning curve prediction to skip bad models~\citep{Baker17}, predicting the accuracies of models before training~\citep{Deng17}, using iterative search method for architectures of growing complexity~\citep{Liu17,Elsken17}, or using hierarchical representation of architectures~\citep{Liu17b}. Our method is also inspired by the concept of weight inheritance in neuro-evolution, which has been demonstrated to have positive effects at scale~\citep{Real17}.

Closely related to our method are other recent approaches that avoid training each architecture from scratch, such as convolutional neural fabrics -- ConvFabrics~\citep{conv_fabrics} and SMASH~\citep{smash_net}. These methods are more computationally efficient than standard NAS. However, the search space of ConvFabrics is not flexible enough to include novel architectures, e.g. architectures with arbitrary skip connections as in~\cite{nas}. Meanwhile, SMASH can design interesting architectures but requires a hypernetwork~\citep{hyper_net} to generate the weights, conditional on the architectures. While a hypernetwork can efficiently \textit{rank} different architectures, as shown in the paper, the real performance of each network is different from its performance with parameters generated by a hypernetwork. Such discrepancy in SMASH can cause misleading signals for reinforcement learning. Even more closely related to our method is PathNet~\citep{fernando2017pathnet}, which uses evolution to search for a path inside a large model for transfer learning between Atari games.


%These methods are either more expensive or design less accurate models compared to our methods.  

% In this work, we propose a novel approach that combines the strengths of both ConvFabrics and SMASH. Unlike SMASH, we do not use a hypernetwork to generate $\omega_\m$ for each $\m$, but instead keep a shared set of parameters $\omega$ among all architectures $\m$. Unlike ConvFabrics, we design a different mechanism to specify computing paths in our model, leading to a very flexible search space. In fact, our search space is larger than the search space of SMASH as well as the search space described in~\cite{nas}. As a result, our method can efficiently discover novel architectures that achieve better accuracy than SMASH.

% Our work is related to several directions in the existing literature. First, we
% show that how all existing approaches for NAS can be viewed as an instance of
% the Bayesian framework that we describe in Section~\ref{sec:methods}. Then, we
% review existing attempts to establish theoretical grounds for NAS.
% 
% \subsection{\label{sec:existing}Approaches for Neural Architecture Search}
% Existing methods for NAS can be classified into two categories. The first
% category of algorithms attempt to design the the architecture of the whole
% network, e.g.  how many channels to use at each convolutional layers, which
% layers should be sent to which layers via residual connections~\cite{res_net},
% etc. Example algorithms of this approach include~\cite{nas} and
% ~\cite{nas_dqn}.  The second category aims to design several particular modules
% and replicate it multiple times to form a model.  Examples of this category
% include~\cite{nas_module}, where the authors attempt to learn convolutional
% modules and pooling modules to build their networks; and~\cite{nas_module_dqn},
% where the authors use a deep Q-network instead of policy gradient to design
% their convolutional modules.~\cite{nas} also contribute an approach to learn
% the formula for a recurrent neural network cell, which is replicated through
% multiple time steps.
% 
% All the approaches mentioned in the previous paragraphs strives to model the
% distribution above possible architectures in their corresponding search space,
% i.e. $q(\m)$ in Eqn.~\ref{eqn:models_and_params}. The parameter distribution
% $q(\theta_\m | \m)$ is not explicitly modeled, and $\theta_\m$ is learned by
% minimizing a cross-entropy loss objective $\theta_\m = \arg\min_{\theta}
% \mathcal{L(\m, \theta)}$.
% 
% Similar approaches such as~\cite{fractal_net,conv_fabrics} and~\cite{smash_net}
% tries to anneal the running time by designing different choices of $q(\m)$ and
% $q(\theta_\m | \m)$.
% 
% Another inspiring method is to derive architectures via Reproduced Kernel
% Hilbert Space (RKHS)~\cite{kernel_nas}.
% 
% 
% \subsection{\label{sec:theory}Existing Theory}
% There are extremely few theory papers on this NAS.
% Recently,~\cite{non_parametric_net} shows that the optimization process has a
% global minimal. More recently,~\cite{ada_net} prove that the Rademacher
% complexity of the set of models is not significantly larger than that of a
% single model, suggesting an easy optimization problem.



